Measures of Tractography Convergence

In the present work, we use information theory to understand the empirical convergence rate of tractography, a widely-used approach to reconstruct anatomical fiber pathways in the living brain. Based on diffusion MRI data, tractography is the starting point for many methods to study brain connectivity. Of the available methods to perform tractography, most reconstruct a finite set of streamlines, or 3D curves, representing probable connections between anatomical regions, yet relatively little is known about how the sampling of this set of streamlines affects downstream results, and how exhaustive the sampling should be. Here we provide a method to measure the information theoretic surprise (self-cross entropy) for tract sampling schema. We then empirically assess four streamline methods. We demonstrate that the relative information gain is very low after a moderate number of streamlines have been generated for each tested method. The results give rise to several guidelines for optimal sampling in brain connectivity analyses.

==> intro/thought_ex.tex <==


To perform streamline tractography is to sample from a distribution of possible tracts through simulation. Diffusion MRI cannot directly observe white matter fascicles; \BlueComment{the unit of observation is a q-space measurement of diffusion propensity for given gradient angles}. Researchers simulate fascicle trajectories from fitted local models, which have parameters estimated from the diffusion signal (for reference and review, see Sotiropoulos and Zalesky \cite{zalesky2017howwhybut})

While for many purposes direct observations would be convenient, the fact that streamline methods are simulations give such generating processes properties that observational data do not have (for which we give evidence afterwards):
\begin{enumerate}
\item Researchers can sample as many streamlines as disk space/computation allow. Moreover, the researcher has complete control over the number of tracts he or she chooses to sample. \label{enm:many_samps}
\item Most common \CiteNeeded streamline methods produce truly i.i.d. samples up to seed point selection; the trajectory one streamline does not affect the next streamline computed, except for seeding choice. \label{enm:iid}
\item Simply because a streamline is biologically implausible does not necessarily invalidate the data generating process \label{enm:noise}.
\end{enumerate}

The first property is clearly true. Nothing prevents the researcher from running a tracking method for months until he or she runs out of disk space, or as many or as few times as he or she wishes.

The second property may be illustrated by the following thought experiment: fix a seed point and run a tracking method twice using that seed point. Regardless of the general method type (probabilistic, deterministic) or local model, the trajectory of second streamline generated does not depend on the first. In the same way we could generate two whole brain tractographies (tractograms) twice on the same scan, and the two would be independent. Further, since nothing has changed between the underlying scan, the local model fits, nor the tracking method, it is safe to assume that both streamlines are drawn from the same distribution (given the seed point). This holds true for a wide variety of streamline algorithms, indeed any that could fit a ``input data and a seed, output a track'' template. \BlueComment{We should provide notable exceptions, if there are any.}.

The third property is the crux of the matter, and we illustrate it by continuing our thought experiment: Consider a tractography method that when queried ten times generates complete noise\footnote{the definition of complete noise is actually tricky, but we could use a proxy of ``drawing a tract length uniformly at random between 1 and the number of voxels, and filling its sequence with points drawn uniformly from the domain of the image''.}
nine times and generates a real tract one time. Clearly this method has high noise ($90\%$ useless!) and would not do well in major tractography challenges (e.g. \cite{maier2017challenge}), but, we claim, this method still has high value. Since the number of real tracts is finite and the number of possible noise tracts is comparatively large, increasing the sample size will lead to each real tract having more corresponding samples than the noise tracts. Given enough time and disk space we may recover the set of real tracts.

We could further make a similar hypothetical situation in which the method (for every ten queries) returns eight noise tracts, one real tract, and one tract that is exactly $1$ cm anterior to the left eye. Taking a sufficiently large sample, we might believe that this false mode outside the skull exists. It is important to be able to characterize and differentiate between the first method and the second, as well as between each of the two and a pure-noise case. Clearly their supports (that is, the set of possible tracts generated) are the same; it is the frequency at which we sample specific instances that changes. 

It is also important to know when (i.e. after how many samples) it is possible to sufficiently characterize and differentiate these generating processes. If for two processes this number is large we should consider them similar; if the number is small we know them to be disparate. 

Towards this end we explore two methods for measuring distributions of tracts and differences between distributions of tracts. We assume that similar tracts usually have similar likelihoods, i.e. a smoothness assumption for some definition of closeness, but the provided \BlueComment{methods } are agnostic to the specific choice of similarity. The first method is based on Information Theory and Kernel Density Estimation (KDE), while the second comes from literature on kernel embeddings of probability distributions.
